GIFT-SW: Gaussian noise Injected Fine-Tuning of Salient Weights for LLMs

Parameter Efficient Fine-Tuning (PEFT) methods have gained popularity and democratized the usage of Large Language Models (LLMs). Recent studies have shown that a small subset of weights significantly impacts performance. Based on this observation, we introduce a novel PEFT method, called Gaussian noise Injected Fine Tuning of Salient Weights (GIFT-SW). Our method updates only salient columns, while injecting Gaussian noise into non-salient ones. To identify these columns, we developeda generalized sensitivity metric that extends and unifies metrics from previous studies. Experiments with LLaMA models demonstrate that GIFT-SW outperforms full fine-tuning and modern PEFT methods under the same computational budget. Moreover, GIFT-SW offers practical advantages to recover performance of models subjected to mixed-precision quantization with keeping salient weights in full precision.

==> latex/archive.tex <==
%%%% intro
Modern open-source Large Language Models (LLM) such as LLaMA \cite{touvron2023llama} and Mistral \cite{jiang2023mistral} can successfully perform complex language modeling across various domains. However, to integrate LLMs into real-world applications, fine-tuning for specific tasks is often necessary \cite{bai2022training, li2023starcoder}. Given that LLMs comprise dozens of transformer blocks containing billions of parameters, fully fine-tuning all parameters requires demanding computational and memory costs. Therefore, substantial efforts are focused on developing Parameter-Efficient Fine-Tuning (PEFT) methods which are able to adapt LLMs to particular fields by optimizing only a restricted set of parameters \cite{han2024parameter}.

 Among PEFT methods, Low-Rank Adaptation (LoRA) \cite{hu2021lora} is the most widely used in industrial applications. According to the approach, low-rank adapters are trained for the selected model layers which weights remains unchanged. Often, the adapters can well approximate the specified sub-task, so the model achieves an acceptable level of specialization. However, for complex tasks, LoRA fine-tuning may not provide the same level of accuracy as full fine-tuning \cite{nikdan2024rosa}. Therefore, novel PEFT methods are proposed to provide high generative performance of models as after full fine-tuning but for modest resources.

In this paper, we investigate a novel PEFT method designed to update outlier columns within weight matrices of LLM. Previous studies related to Post-Training Quantization \cite{dettmers2022gpt3, dettmers2023spqr, kim2023squeezellm} have shown the substantial contribution of outlier weights and activations to the quantization error of LLMs. Therefore, the hybrid quantization schemes, which isolate outliers from weights being quantized, enable to improve quantization performance. Additionally, it has been observed that rather than extracting sparse outliers, only the columns, which are the most sensitive to quantization, can be stored in high-precision. On the other hand, ~\citeposs{yin2023outlier} demonstrated that the effectiveness of advance pruning methods SparseGPT
\cite{frantar2023sparsegpt} and Wanda \cite{sun2023simple} is also related to the carefully retention of outlier weights. On the basis of the mentioned studies, it can be concluded that the generative capabilities of modern LLMs highly depends on outliers.

On the basis of the mentioned studies, it can be concluded that the generative capabilities of modern LLMs highly depends on outliers. Following to the conclusion, we adopt fine-tuning of outlier columns to enhance original pre-trained LLMs with limited computational budgets. Since outlier columns persist after quantization at high precision, this method naturally can be applied to restoring the quality of quantized models. Previously, Weak Column Tuning included in OWQ \cite{lee2024owq} showed that training in 4bit quantized model only columns with outliers gives accuracy comparable with LoRA. To explore the viability of the approach, we consider different metrics for selection of columns with outliers for quantizing pre-trained models into 2, 3, 4 bits, and train of the chosen columns in weight matrices of the models quantized with GPTQ \cite{frantar2022gptq}.

Moreover, we propose a modification of the fine-tuning of outlier columns in weight matrices by inserting Gaussian noise to other columns. From previous studies of Pertrubed Gradient Descent (PGD) optimization it is well known that noise injections both after and before the gradient step facilitate to stabilization of convergence and prevent overfitting \cite{poole2014analyzing, zhu2018anisotropic, jin2021nonconvex}. On the other hand, pre-training of a model with noise enable to approximate quantization error \cite{shvetsov2022quantnas, shin2023nipq}. As a result, the pre-trained model is prepared to weights quantization and better preserves prediction capabilities. According to this studies, we determine noise magnitude based on quantization scale and show that noise insertion improves fine-tuning of outlier columns.


%%%% PEft
The approach was successfully adapted and modified for PEFT of quantized LLMs such that QLoRA [Dettmers, T., Pagnoni, A., Holtzman, A., & Zettlemoyer, L. (2024). Qlora: Efficient finetuning of quantized llms. Advances in Neural Information Processing Systems, 36.], LoftQ [Li, Y., Yu, Y., Liang, C., He, P., Karampatziakis, N., Chen, W., & Zhao, T. (2023). Loftq: Lora-fine-tuning-aware quantization for large language models. arXiv preprint arXiv:2310.08659.], LQ-LoRA [Guo, H., Greengard, P., Xing, E. P., & Kim, Y. (2023). Lq-lora: Low-rank plus quantized matrix decomposition for efficient language model finetuning. arXiv preprint arXiv:2311.12023.], IR-QLoRA [Qin, H., Ma, X., Zheng, X., Li, X., Zhang, Y., Liu, S., ... & Magno, M. (2024). Accurate LoRA-Finetuning Quantization of LLMs via Information Retention. arXiv preprint arXiv:2402.05445.], ApiQ [Liao, B., & Monz, C. (2024). ApiQ: Finetuning of 2-Bit Quantized Large Language Model. arXiv preprint arXiv:2402.05147.]. Other approaches for quantized models directed to fine-tuning of quantization scales, zeros and weight clipping thresholds [Kim, J., Lee, J. H., Kim, S., Park, J., Yoo, K. M., Kwon, S. J., & Lee, D. (2024). Memory-efficient fine-tuning of compressed large language models via sub-4-bit integer quantization. Advances in Neural Information Processing Systems, 36., Shao, W., Chen, M., Zhang, Z., Xu, P., Zhao, L., Li, Z., ... & Luo, P. (2023). Omniquant: Omnidirectionally calibrated quantization for large language models. arXiv preprint arXiv:2308.13137.], tweaking parameters in LayerNorm layers [Li, L., Li, Q., Zhang, B., & Chu, X. (2024, March). Norm tweaking: High-performance low-bit quantization of large language models. In Proceedings of the AAAI Conference on Artificial Intelligence (Vol. 38, No. 17, pp. 18536-18544).]. In comparison with LoRA-based schemes, these methods are more cost-efficient, but unable to achieve high accuracy.
Experiments on quantization methods of LLMs well established that outlier values in weights and activations have a significant impact on prediction quality. Therefore, fine-tuning low number of weight outliers can be a promising approach for recovering accuracy of quantized models without the need for high memory requirements and the insertion of additional layers. OWQ [Lee, C., Jin, J., Kim, T., Kim, H., & Park, E. (2023). Owq: Lessons learned from activation outliers for weight quantization in large language models. arXiv preprint arXiv:2306.02272.] combined with training of columns with weight outliers surpasses QLoRA and yields results comparable with LoRA. The present paper focuses on detail investigation of an influence of different kind of columns with outliers on accuracy of open-source LLMs after quantization and their sensitivity to fine-tuning based on modern instructive datasets.

%%%% outlier selection background
An important challenge for Post-Training Quantization of LLMs is outlier values in weight and activation matrices. ~\citeposs{dettmers2022gpt3} showed that the outliers in activation greatly impact on predictive performance of large transformers. To support the accuracy of quantized model, the authors developed LLM.int8() for int8 weights and activation quantization where the features with outliers are isolated from regular values during inference (\textbf{forward pass?}). ~\citeposs{xiao2023smoothquant} showed that the outliers in activations appear in small fraction of channels. Based on the observation, SmoothQuant was proposed where the outlier values in activation are found offline using a small calibration dataset and their magnitudes are smoothed with per-channel scaling transformation. By adopting the similar outlier selection procedure, QUIK \cite{ashkboos2023quik} keeps activations containing columns with outliers and corresponding weight columns in floating point data types, while other columns are quantized with applying of GPTQ. 

In the context of only weight quantization OWQ \cite{lee2024owq} incorporates the same approach, but with different identification of columns with outliers based on the quantization error and sensitivity measure provided by OBD (Optimal Brain Damage) \cite{lecun1989optimal}. SpQR \cite{dettmers2023spqr} modifies GPTQ \cite{} by excluding from the quantization process unstructured sparse outliers in weights, which are found by using metric given by the OBC (Optimal Brain Compression) framework \cite{frantar2022optimal}. Another method extracting sparse outliers in weight is SqueezeLLM \cite{kim2023squeezellm} where the outliers are identified based on the weight magnitudes and quantization is conducted in non-uniform configuration accounting for weight distribution. Also, QuantEase \cite{behdin2023quantease} includes procedure with the proximal gradient method to find unstructured or structural outliers in weights. 

%%%quant error

For a linear layer of the model, let $\mathbf{X} \in \mathbb{R}^{C_{in}\times N}$ is the input feature and  $\mathbf{W} \in \mathbb{R}^{C_{out}\times C_{in}}$ is the full-precision weight matrix, where $C_{in}$ and $C_{out}$ represents the number of the input and output channels, $N$ is the sequence length of the input. Then in the layer-wise quantization the quantized weight $\tilde{\mathbf{W}} \in \mathbb{R}^{C_{out}\times C_{in}}$ is found to minimize the objective function
\begin{equation}
  \label{eq:layerwise_quant_error}
  \mathrm{argmin}_{\tilde{\mathbf{W}}} \Vert \mathbf{W} \mathbf{X} - \tilde{\mathbf{W}} \mathbf{X} \Vert_{2}^{2}.
\end{equation}
The function captures the distance between the outputs with original and quantized weights.

%%%%%% gaussian noise

As can be seen from Eq. \ref{eq:gni_finetuning}, the Gaussian noise is injected only into the non-trainable parameters, whereas outlier columns are trained as usual without noise. According to the sensitivity metrics presented in the previous section, quantization of the outlier columns induces a significant quantization error. Therefore, the parameters computed accounting for the outliers leads to high quantization noise which complicates the training due to large shifting of the frozen weights. Moreover, deviation of outliers from the original state can irreversibly disrupt the predictive capabilities of the model.   

%%%%% gptq

In the present study quantization framework of LLMs is based on the GPTQ method. It is a PTQ method, which conducts weight only uniform layer-wise quantization with error compensation using the Hessian information. The layer-wise quantization process is derived for each layer from the optimization problem.

According to GPTQ, quantization of the weight matrix  $\mathbf{W}$ is performed iteratively column by column. Weights $\mathbf{W}_{:, j}$ in a column $j$ are quantized simultaneously. To reduce the error Eq.\ref{eq:layerwise_quant_error}, the remaining full-precision weights $\mathbf{W}_{:, j:}$ are updated. The optimal weights update is determined based on the OBS theory:



\begin{equation}
  \label{eq:obs_weight_update}
\mathbf{W}_{:, j:} \leftarrow  \mathbf{W}_{:, j:} - \frac{(\mathbf{W}_{:, j} - \tilde{\mathbf{W}}_{:, j})}{[\mathbf{H}^{-1}]_{jj}}\mathbf{H}^{-1}_{j,j:},
\end{equation}

where $\mathbf{H} = 2\mathbf{X}\mathbf{X}^{T}$ is Hessian corresponding to Eq.\ref{eq:layerwise_quant_error}. 

To improve computational efficiency, GPTQ adopts a lazy-batch update scheme. This means that quantization with error compensation is performed through blocks of columns (usually 128 columns at a time). As a result, the weights are only updated in a subset of columns.

%%%%% sensitivity metrics
First, we describe our generalized criterion and then discuss how it connects to the previous results. 
We focus on selecting a column with the highest number of outliers, first we compute $s_{j}$ for each column as in Equation~\ref{eq:general} and then select a small subset of columns with the highest values.  Here $\tilde{\mathbf{W}}$ denotes perturbed weights. Since we previously established connection between Gaussian noise and quantization noise we can easily apply methods developed for perturbed via quantization weights, which are studied in the recent literature on quantization. In other words, we choose columns which are most sensitive to noise perturbations. 


First, we presents the metrics in a generalized view. Then we discuss metrics proposed in the previous mixed-precision quantization methods.

As it is mentioned in theprevious Section, injection of quantization noise into weights simulates their quantization. Therefore, to find columns which are highly corrupted by the noise, we adopt sensitivity metrics which shows an impact of quantizaion on weights of columns. First, we describe our generalized criterion. Then discuss how it connects to metrics proposed in the previous mixed-precision quantization methods.


Therefore, columns that are highly corrupted by noise can be identified using sensitivity metrics designed to predict the impact of quantization on the weights of the columns.

\begin{equation}
  s_{j} = \Vert \mathbf{W}_{:, j} - \tilde{\mathbf{W}}_{:, j} \Vert_{\Upsilon}^{\beta} \Vert \mathbf{X}_{:, j} \Vert_{\Upsilon}^{\gamma}
  \label{eq:general}
\end{equation}

Here we consider following values for the parameters above $\beta \in \{0,1,2 \}$, $\gamma \in \{0,1,2 \}$ and $\Upsilon \in \{L_2,L_{\inf} \}$. Choice of these values is based on the observations of criterions from previous papers and our own assumptions.

We compute $s_{j}$ for each column of the matrix $\mathbf{W}$ and then select a small subset of columns with the highest values.

It can be seen that the cases $\gamma = 1$ and $\gamma = 2$ give the influence of the input activation on the sensitivity metric similar to Quik and OWQ. To study another relationship between the weights deviation and the input activation $\gamma = 1/2$ is considered. 

In QUIK following to SmoothQuant outlier columns in weight matrix are selected based on $l_{\infty}$ norm computed for the corresponding columns of the input feature $\mathbf{X}$. In this case the sensitivity metric for $j$-th column is written as

\begin{equation}
  \label{eq:quik_metric}
  s_{j} = \Vert \mathbf{X}_{:, j} \Vert_{\infty},
\end{equation}
which corresponds to the set $\beta \gamma \Upsilon = (0,1, \inf)$.

The proposed metric Eq. \ref{eq:our_metric} is closely related to those studied in the recent literature on quantization. If we take only $l_{\infty}$ norm of the input features $\mathbf{X}$ with $\gamma=1$, then Eq. \ref{eq:our_metric} turns out to the metric $\Vert \mathbf{X}\Vert_{\infty}$  employed in QUIK \cite{ashkboos2023quik} and SmoothQuant \cite{xiao2023smoothquant}. If we adopt $l_{2}$ norm for the weight error and the input feature with $\gamma=2$, then the metric is written as $\lambda_{j}\Vert \mathbf{W}_{:, j} - Q(\mathbf{W}_{:, j})\Vert_{2}^{2}$, where $\lambda_{j} = \Vert \mathbf{X} \Vert_{2}^{2}$ is the $j$-th diagonal element of the Hessian matrix $\mathbf{H}$ for the layer quantization error


In OWQ the sensitivity metric is defined  accounting for the Hessian matrix $\mathbf{H}$ as in OBS~\cite{frantar2023sparsegpt, frantar2022gptq}, and perturbation of weights in columns induced by the quantization. For $j$-th weight column the metric is written as 

\begin{equation}
  \label{eq:owq_metric}
  s_{j} = \lambda_{j} \Vert \mathbf{W}_{:, j} - \tilde{\mathbf{W}}_{:, j} \Vert_{2}^{2},
\end{equation}

where $\lambda_{j} = \mathrm{diag}(\mathbf{X}\mathbf_{X})_{j}$ is the $j$-th diagonal element of the Hessian matrix $\mathbf{H}$ for the layer quantization error Eq. \ref{eq:layerwise_quant_error}. 

==> latex/archive_abstract.tex <==
Parameter Efficient Fine-Tuning (PEFT) methods have gained popularity and democratized the usage of Large Language Models (LLMs). Typically, PEFT methods require to insert low-rank or other adapters into LLM layers. However, recent studies on quantization and pruning reveal that there is a subset of salient weights within neural networks whose perturbations highly affect overall model performance. Based on this observation, we introduce a novel PEFT method, called Salient Columns Fine-tuning with Quantization Noise Injection (\naming{}). Our method updates weights in salient columns while injecting quantization noise into the non-salient weights during each iteration, analogous to the Perturbed Gradient Descent technique. The noise injection purposes to improve the generalization capabilities of the salient weights. To identify salient columns, we derive sensitive metrics, that are applied to pre-trained models prior to the fine-tuning process. Experiments with original LLaMA2 \& 3 demonstrate that \naming{} outperforms full fine-tuning and contemporary PEFT methods under the same computational budget.  Furthermore, when applied to quantized LLaMA models, \naming{} can recover model quality better than the straight-through estimators.

==> latex/archive_background.tex <==
\section{Background and Related Work}
\subsection{Parameter efficient fine-tuning of LLM}
One of the most popular method with high efficiency is LoRA \cite{hu2021lora} which trains the low-rank adapters for layers of the pretrained model. Recent modifications to the method aim to improve the initialization of the adapters \cite{liu2024dora} and enhance the low-rank representation of pre-trained weights by adding a sparse adapter \cite{nikdan2024rosa}. Also, LoRA was successfully adapted and modified for PEFT of quantized LLMs such that QLoRA \cite{dettmers2024qlora}, LoftQ \cite{li2023loftq}, LQ-LoRA \cite{guo2023lq}.

\textcolor{blue}{Although LoRA and its various modifications are widely used in industry to specialize pre-trained models for downstream tasks and recover the accuracy of quantized models, we claim that a small number of weight outliers may be manageable to fine-tuning. }

% \citeauthor{lee2024owq} showed that training of outlier columns in LLaMA-7B quantized with OWQ in 4 bit surpasses QLoRA and yields results comparable with LoRA.





\subsection{LLM quantization and outliers\protect\footnote{In our work, we use the terms \textbf{outliers} and \textbf{salient weights} interchangeably. However, we believe that the latter term is more suitable.} importance}

There are two primary approaches for Post-Training Quantization (PTQ) for Large LLMs: Joint weight-activation quantization and only weight quantization methods. Our focus lies within the latter category. Both approaches encounter a significant challenge posed by outlier values present in weight and activation matrices.

\textit{Joint weight-activation quantization:} \citeposs{dettmers2022gpt3} demonstrated that a small subset of activations has a substantial impact on LLM performance. The authors introduced LLM.int8(), a method for int8 weights and activation quantization, which isolates features with outliers from regular values. \citeposs{xiao2023smoothquant} work further revealed that outliers in activations are confined to a small fraction of channels. This insight led to the development of SmoothQuant, a method that identifies outlier values in activations offline using a small calibration dataset and smooths their magnitudes with per-channel scaling transformation.
Similarly, QUIK~\cite{ashkboos2023quik} retains activations containing columns with outliers and corresponding weight columns in floating point data types, while other columns are quantized using the GPTQ~\citep{frantar2022gptq} approach. 

\textit{Only weight quantization:} In this context,  OWQ~\cite{lee2024owq} incorporates a similar approach by splitting outlier and non outlier weights into different matrices but employs a different method for identifying columns with outliers based on quantization error and sensitivity measures provided by Optimal Brain Damage \citep{lecun1989optimal}. In SpQR~\cite{dettmers2023spqr} authors proposed to exclude unstructured  outliers and keep them in a sparse matrix  instead of columns, which is more flexible. Outlier weights are identified using metrics from the Optimal Brain Compression (OBC)~\cite{frantar2022optimal} framework.

In SqueezeLLM \cite{kim2023squeezellm} weights are also separated into a sparse matrix, however,  the outliers are identified based on the weight magnitudes and in contrast to above methods non-uniform quantization is applied. QuantEase \cite{behdin2023quantease} poses weight outlier identification as an optimization problem and solves it  with the proximal gradient method.



\subsection{Gaussian Noise Injections (GNI)}
\textbf{Pertrubed Gradient Descent (PGD)} is a family of methods that involve adding or multiplying samples from some  noise distribution, during optimization procedure. \textbf{PGD} has a strong theoretical support. Noise injections \textit{after the gradient step}: $\mathbf{W}_{t+1} \leftarrow \mathbf{W}_{t} - \tau (\nabla f(\mathbf{W}_{t}) + \mathbf{\xi})$ allow to escape saddle points efficiently in non-convex optimization~\citep{jin2021nonconvex}. And if applied \textit{before the gradient step}: $\mathbf{W}_{t+1} \leftarrow \mathbf{W}_{t} - \tau (\nabla f(\mathbf{W}_{t} + \mathbf{\xi})  )$  help to escape from the spurious local optimum~\citep{zhu2018anisotropic}. Noise in both cases is sampled from normal distribution $\mathbf{\xi} \sim \mathcal{N}(\mu,\,\sigma^{2})$~\footnote{Each parameter of $\xi$ is sampled from standard normal distribution}.  In the convex case, this is typically
used to smooth a non-smooth objective function \cite{duchi2012randomized, jin2017escape}.

% \begin{align}
%     \label{eq:pgd_one} \theta_{t+1} \leftarrow \theta_{t} - \tau (\nabla f(\theta_{t}) + \xi) \\\ 
%     \label{eq:pgd_two} \theta_{t+1} \leftarrow \theta_{t} - \tau (\nabla f(\theta_{t} + \xi)  ) \\
%     \xi \sim \mathcal{N}(\mu,\,\sigma^{2})  
% \end{align}

Practical benefits of noise injections are well documented in the literature and often can be discussed as regularization techniques~\cite{bishop1995training, srivastava2014dropout, camuto2020explicit}, methods to prompt adversarial robustenss~\cite{panda2021implicit} and to be used for data agumentation~\cite{moreno2018forward}.
%\egor{need to highlight that it is documented but not commonly used in practice for some reason}


Models trained with noise often generalise better to unseen data and are less prone to overfitting~\cite{srivastava2014dropout, poole2014analyzing}. They have wider (smoother) minima, lesser sensitivity to perturbations, and better calibration~\cite{camuto2020explicit}. 

 % There are two options for injecting the noise: adding perturbations \textit{after each gradient descent step} (equation~\ref{eq:pgd_one}) or adding perturbations to the iterate \textit{before evaluating the gradient} equation~\ref{eq:pgd_two}. 
 
 In our work we use GNI applied \textit{before evaluating the gradient}. \citet{orvieto2023explicit} empirically and theoretically demonstrated that GNI in such scenario can be used as a regularization and proposed to add noise only to one layer at a time to avoid variance explosion.   % However, in contrast to our work empirical results are obtained for full model training and to relatively small models. 
 \citet{liu2023pac} studied fine-tuning of Pre-trained Language Models with GNI, authors proposed first to learn layer-wise variance parameters for noise distributions and then to fine-tune the model by adding noise to all the weights. They demonstrated that their approach is superior to independent layer-wise noise injections proposed by \citet{orvieto2023explicit}. 
 
 
%  While the benefits of Projected Gradient Descent (PGD) are well-studied in the literature, its application to Large Language Models (LLMs) is limited. Only one work has studied the fine-tuning of Pre-trained Language Models (PLMs) with PGD, where the authors proposed a modification of PGD that first learns layer-wise variance parameters 
% .

 %The so-perturbed gradient is then used to update the unperturbed iterate. 


% In our work we apply additive to weights noise to all the weights, except to the group of salient weights. It is important to note, that additive to weights noise can be regarded as multiplicative to activations noise and since we do not want to corrupt signal from salient weights we use additive to weights strategy. 


\subsection{Quantization Noise Injections (QNI)}
Uniform quantization~\footnote{For the reader not familiar with uniform quantization we discuss it in more details in Section~\ref{appendix:uniform quantization}.} - $Q(\cdot)$ is a non differentiable operation, if simplified it can be expressed as a composition of scaling and rounding operations, $Q(\mathbf{W})=\round{\frac{\mathbf{W}}{s}}$.    It has been shown that in terms of quantization aware training, quantization operation can be efficiently approximated with quantization noise ~\cite{defossez2021differentiable, shvetsov2022quantnas, shin2023nipq} such that  $\Omega = \round{\frac{\mathbf{W}}{s}} - \mathbf{W}$, which is exactly the same as training models with GNI, if we assume that $\Omega$ and $\xi$ have identical distributions. Under some assumptions the effect of uniform quantization can often be modeled by an additive noise that is uniformly distributed, uncorrelated with the input signal,  and has a white spectrum \cite{widrow1996statistical}. In practice, these assumptions, usually do not hold true, and assuming that $\Omega \sim \mathcal{N}(\mu,\,\sigma^{2})$ comes from Gaussian distribution leads to better results \cite{defossez2021differentiable, shvetsov2022quantnas}. \

% \begin{align}
%     \label {eq:quant} Q(\theta) = \round{\frac{\theta}{s}} \\
%     \label {eq:noise} \Omega = \round{\frac{\theta}{s}} - \theta   \\
%     \Omega \sim \mathcal{N}(\mu,\,\sigma^{2})  \\
%     \label{eq:quant_noise} \theta_{t+1} \leftarrow \theta_{t} - \tau (\nabla f(\theta_{t} +  \Omega ) 
% \end{align}

\subsection{Straight Through Estimator}
Quantization is inherently a non-differentiable operation, therefore, we need to employ an approximation to incorporate it into the training process. Straight Through Estimation (STE)\footnote{More details on STE can be found in Section~\ref{appendix: STE}.}~\cite{bengio2013estimating} is commonly used for that, which is basically re-parameterizes gradients.  \citeposs{defossez2021differentiable} demonstrated that STE has some disadvantages compared with QNI\footnote{Event though QNI and GNI are identical operations for consistency and clarity,  in the case of quantization we will refer to this procedure as Quantization Noise Injections (QNI)}, STE is biased and may cause weight oscillation between quantization steps.  \citeposs{shin2023nipq} demonstrated that pretraining models for the following quantization with QNI instead of STE results in better performance and \citeposs{shvetsov2022quantnas} used QNI to search for quantization friendly neural architectures, approximating model degradation caused bu quantization with QNI.

% \textcolor{blue}{In this work, we study model fine-tuning with QNI for the following quantization, and demonstrate that QNI is advantageous for the following quantization and depends on a choice of quantization step.}

==> latex/archive_e.tex <==
%% method
GIFT-SW employs fine-tuning  salient columns with noise injection. The method consists of the following steps:
 \vspace{-2mm}
\begin{itemize}
\setlength\itemsep{0em}
\item[(1)] Identify a small number of columns with the highest concentration of salient weights using a chosen metric. We cover the choice of metrics in Section~\ref{sec:metrics}.  \vspace{-2mm}
\item[(2)] Split the matrices into two subsets: one for salient weights and one for non-salient weights.  \vspace{-2mm}
\item[(3)] During training, add noise to the non-salient weights and update only the salient weights. We discuss noise injection details in Section~\ref{sec:noise}. In the case of quantization, quantize the non-salient weights while keeping the salient weights with their initial precision.  \vspace{-2mm}
\end{itemize}
    

% In this section we propose our PEFT method for LLMs which trains outliers with Gaussian noise injection. As it is mentioned in \cite{yin2023outlier, puccetti2022outliers}, outlier values in weights of modern LLMs are responsible for high predictive performance of modern LLMs. At the same time, the weights with a large range are difficult for low-bits quantization, as it is not possible to find a suitable scaling factor within the framework of linear quantization. Therefore, outliers retention is a promising way to improve quality of sparse and quantized models. But in the present work, we also show that the outliers can be efficiently employed for fine-tuning. 

% Instead of isolating outliers into sparse matrix,  we select columns with outliers. According to OWQ and Quik, there is a great potential for efficient implementation on GPUs  with low runtime and memory overhead.

% Since identifying outlier columns at runtime dynamically increases the consumption of computational resources, we select the subset of columns for each layer before fine-tuning or quantization using a calibration set. 


We select the subset of columns for each layer before fine-tuning or quantization using a small calibration set. We use a fixed number of columns for each layer, more technical details can be found in Section~\ref{sec:exps}. Based on results from the previous works we assume that salient weights do not change during fine-tuning, however, this assumption requires further investigation and out of the scope of our work. Additionally, we tried adaptive schemes to allocate different number of columns to each layer proportional to the number of salient weights and we did not observe any improvements, so we do not present these results here and use fixed number for each column. 

An important component of our method is a criteria for identifying outlier columns. In Section~\ref{sec:metrics} we generalize previously studied metrics provided by QUIK~\cite{ashkboos2023quik} and OWQ~\cite{lee2024owq}, and propose our modifications. 

%%

==> latex/discussion.tex <==
\section{Discussion}


We pose a question for the further research if we update the same salient weights with and can we consider these procedures to be equivalent. 

Another related questions if "universal neurones" present the same or similar subset of weights as salient weights.

Can we further improve noise injected fine-tuning? We did not look into that part deeply.

==> latex/outlier_ablation_archive.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{llccccc}
        \hline
        \multirow{2}{*}{Bits} & \multirow{2}{*}{Model} & \multicolumn{5}{c}{Sensitive metric} \\
        \cline{3-7}
         & & $\Vert \mathbf{D}_{j} \Vert_{\infty} \Vert \mathbf{X}_{j} \Vert_{\infty}^{\gamma}$ & $\gamma=1$ & QUIK & $\gamma=1/2$ & $\gamma=2$ \\
        \midrule
        \multirow{4}{*}{4 bit} 
         & LLaMA2-7b & $\mathbf{69.86}$ & $69.85$ & $69.68$ & $69.55$ & $69.52$ \\
         & T\"ULU2-7b & $72.94$ & $\mathbf{73.17}$ & $72.77$ & $72.22$ &  $72.78$ \\
         \cline{2-7}
         & LLaMA2-13b & $72.92$ & $\mathbf{72.99}$ & $72.83$ & $72.83$ & $72.56$ \\
         & T\"ULU2-13b & $75.12$ & $74.86$ & $ 75.19$ & $\mathbf{75.47}$ & $75.17$ \\
        \midrule
        \multirow{4}{*}{3 bit} 
         & LLaMA2-7b & $67.50$ & $\mathbf{68.31}$ & $67.47$ & $68.09$ & $67.86$ \\
          & T\"ULU2-7b & $70.91$ & $\mathbf{71.30}$ & $70.85$ & $71.14$ & $70.88$ \\
          \cline{2-7}
         & LLaMA2-13b & $71.92$ & $71.59$ & $\mathbf{72.10}$ & $71.77$ & $71.45$ \\
         & T\"ULU2-13b & $\mathbf{74.33}$ & $74.07$ & $74.07$ & $74.09$ & $74.31$ \\
        \midrule
        \multirow{4}{*}{2 bit} 
         & LLaMA2-7b & $45.86$ & $46.78$ & $45.99$ & $46.81$ & $\mathbf{46.83}$ \\
         & T\"ULU2-7b & $\mathbf{54.84}$ & $46.85$ & $46.78$ & $48.56$ & $48.20$ \\
         \cline{2-7}
         & LLaMA2-13b & $57.07$ & $\mathbf{57.36}$ & $51.83$ & $57.30$ & $56.73$ \\
         & T\"ULU2-13b & $59.62$ & $59.62$ & $59.43$ & $\mathbf{60.67}$ & $59.39$ \\
        \hline
    \end{tabular}
    \caption{Performance of LLaMA2 and T\"ULU2 models \textcolor{cyan}{after QUIK weight only quantization} with various salient columns selected with metrics of OWQ, QUIK, and Equation \ref{eq:our_metric}. $D_{j} = \mathbf{W}_{:, j} - Q(\mathbf{W}_{:, j})$} 
    \label{tab:outlier_ablation}
\end{table*}
